Visual Program Distillation: Distilling Tools and Programmatic Reasoning into Vision-Language Models

Solving complex visual tasks such as "Who invented the musical instrument on the right?" involves a composition of skills: understanding space, recognizing instruments, and also retrieving prior knowledge. Recent work shows promise by decomposing such tasks using a large language model (LLM) into an executable program that invokes specialized vision models. However, generated programs are error-prone: they omit necessary steps, include spurious ones, and are unable to recover when the specialized models give incorrect outputs. Moreover, they require loading multiple models, incurring high latency and computation costs. We propose Visual Program Distillation (VPD), an instruction tuning framework that produces a vision-language model (VLM) capable of solving complex visual tasks with a single forward pass. VPD distills the reasoning ability of LLMs by using them to sample multiple candidate programs, which are then executed and verified to identify a correct one. It translates each correct program into a language description of the reasoning steps, which are then distilled into a VLM. Extensive experiments show that VPD improves the VLM's ability to count, understand spatial relations, and reason compositionally. Our VPD-trained PaLI-X outperforms all prior VLMs, achieving state-of-the-art performance across complex vision tasks, including MMBench, OK-VQA, A-OKVQA, TallyQA, POPE, and Hateful Memes. An evaluation with human annotators also confirms that VPD improves model response factuality and consistency. Finally, experiments on content moderation demonstrate that VPD is also helpful for adaptation to real-world applications with limited data.

==> old/0_abstract_v0.tex <==



Solving complex visual tasks (e.g., ``Who invented the musical instrument on the right?") involves back-and-forth between visual processing and reasoning. Visual programming, a recent multimodal framework, has shown promise in conducting visual reasoning in an interpretable and compositional manner. Given a query, it first uses a language model (LM) to generate a program, and then executes this program with visual modules to get the answer.
However, this framework is error-prone—it can lead to a wrong answer whenever the program itself is wrong, or when any of the steps of the program are solved incorrectly, thus leading to worse overall performance than end-to-end systems trained with labeled data. Moreover, it is inefficient to involve multiple steps (i.e., generating and then running programs) during inference. Ideally, a single large multimodal model (LMM) should directly conduct similar reasoning and yield the correct answer.
In this work, we propose Visual Program Tuning (VPT), which leverages visual programs for teaching LLMs to reason via instruction tuning. VPT rewrites the execution traces of visual programs as chain-of-thought reasoning steps, and tunes an LMM to output not only the label but its reasoning as well. Extensive experiments on complex vision tasks show that models trained with VPT achieve state-of-the-art accuracy while being able to produce interpretable and faithful reasoning steps. PaLI-X + VPT outperforms all existing LMMs on a wide range of visual tasks, improving performance on counting, spatial relations, and compositional reasoning tasks. VPT is also helpful for quick adaptation on new tasks. Our experiments on content moderation show that fine-tuning LMMs with program-augmented examples is more sample efficient than traditional supervised training.


==> old/0_abstract_v1.tex <==



Solving complex visual tasks (e.g., ``Who invented the musical instrument on the right?'') involves a composition of skills: understanding spatial layouts to focus on the right, recognizing the musical instrument, and accessing prior knowledge to retrieve the inventor. Recent work shows promise by decomposing such tasks using a large language model (LLM) into an executable program with a sequence of invocations to specialized vision models.
However, this procedure is error-prone. Generated programs omit necessary steps or include spurious ones; even if the program is correct, individual model invocations can result in incorrect outputs, from which the overall program never recovers.
Moreover, this inference process requires loading and executing multiple models, incurring high latency and computation cost. 
In this work, we propose Visual Program Distillation (VPD), an instruction tuning framework that produces a vision-language model capable of solving complex visual tasks with a single forward pass.
Given a training dataset of complex visual tasks, VPD first invokes an LLM to generate multiple candidate programs and executes them using visual models to identify a correct program. Next, it translates each code step in the correct program into a natural language description. Finally, it distills this reasoning capability from the LLM into a vision-language model.
Extensive experiments show that our VPD trained PaLI-X achieves state-of-the-art performance across $10$ complex vision benchmarks: VQAv2, GQA, OK-VQA, A-OKVQA, TallyQA, TextVQA, POPE, MMB, VSR, HM.
In addition, VPD models produce human-interpretable and faithful reasoning steps.
Our analysis showcases that VPD models improved capabity for counting, spatial relations, and compositional reasoning. 
VPD can also quickly tune models for real-world applications with limited training data; our experiments on content moderation show that VPD is more sample efficient than traditional supervised training.






%By contrast, the neighboring field of natural language processing finds such decomposition is unnecessary for complex language tasks; with expensive labeled instruction data, a single large language model can be trained to perform all these steps of reasoning within a single forward pass.

 


==> old/0_abstract_v2.tex <==




\begin{abstract}
Solving complex visual tasks such as ``Who invented the musical instrument on the right?'' involves a composition of skills: understanding spatial layouts to focus on the right side, recognizing the musical instrument, and accessing prior knowledge to retrieve the inventor. Recent work shows promise by decomposing such tasks using a large language model (LLM) into an executable program with a sequence of invocations to specialized vision models.
However, this procedure is error-prone. Generated programs may omit necessary steps or include spurious ones; even if the program is correct, individual model invocations can produce incorrect outputs, from which the overall program never recovers.
Moreover, this inference process requires loading and executing multiple models, incurring high latency and computation cost. 
In this work, we propose Visual Program Distillation (VPD), an instruction tuning framework that produces a vision-language model capable of solving complex visual tasks with a single forward pass.
Given a training dataset of complex visual tasks, VPD distills the reasoning capacity within LLMs by sampling multiple candidate programs and executing them to identify the correct one. It translates each correct program into a language description of the reasoning steps, which are then distilled into a vision-language model.
Extensive experiments show that our VPD trained PaLI-X achieves state-of-the-art performance across $10$ complex vision benchmarks: VQAv2, GQA, OK-VQA, A-OKVQA, TallyQA, TextVQA, POPE, MMB,  HM.
In addition, VPD models produce human-interpretable and faithful reasoning steps.
Our analysis showcases that VPD improves model's ability to count, understand spatial relations, and reason compositionally.
% VPD can also quickly tune models for real-world applications with limited training data; our experiments on content moderation show that VPD is more sample efficient than traditional supervised training.

\end{abstract}

\begin{figure}[ht]
\centering
  \includegraphics[width=0.4\textwidth]{figures/radar.png}
  \caption{
We introduce Visual Program Distillation (VPD), which leverages visual programs to generate faithful chain-of-thought training data for Vision-Language Models (VLMs). Our generalist models trained with VPD, \textbf{PaLI-3 VPD (5B)} and \textbf{PaLI-X VPD (55B)}, outperform prior VLMs on a broad range of tasks, while producing human-interpretable and faithful reasoning steps.
\ranjay{Other models are the different color of gray}}
  \vspace{-4mm}
  \label{fig:radar}
\end{figure}


%By contrast, the neighboring field of natural language processing finds such decomposition is unnecessary for complex language tasks; with expensive labeled instruction data, a single large language model can be trained to perform all these steps of reasoning within a single forward pass.

 


==> old/1_intro_v0.tex <==


\begin{figure}[ht]
\centering
  \includegraphics[width=\linewidth]{figures/vpd_demos_fig_outside.pdf}
  \caption{
Outputs of PaLI-X trained with Visual Program Distillation (VPD). PaLI-X VPD is trained with execution traces of filtered programs, and is capable of producing human-interpretable and faithful reasoning steps. This ability also improve model's ability to count, understand spatial relations, and reason compositionally. The images are from Visual Genome.
}
  \vspace{-4mm}
  \label{fig:demo_intro}
\end{figure}


\section{Introduction}
\label{sec:intro}


% Solving complex visual tasks (e.g., ``Who invented the musical instrument on the right?") involves back-and-forth between visual processing and reasoning. Visual programming, a recent multimodal framework, has shown promise in conducting visual reasoning in an interpretable and compositional manner. Given a query, it first uses a language model (LM) to generate a program, and then executes this program with visual modules to get the answer. Nevertheless, this framework easily breaks in practice—for instance, when the program is wrong, or when the visual modules make mistakes in one of the steps of the program. Such error accumulation makes visual programs’ performance much lower than end-to-end systems trained with labeled data. In addition, it is inefficient to involve multiple steps (i.e., generating and then running programs) during inference. An ideal large multimodal model (LMM) should directly conduct similar reasoning and yield the correct answer.

% In this work, we propose Visual Program Tuning (VPT), allowing visual programs to benefit instruction tuning of LMMs: we rewrite the execution traces of visual programs as chain-of-thought reasoning steps, and train LMMs to output not only the label but also these reasoning steps. Extensive experiments on complex vision tasks show that models trained with VPT achieve state-of-the-art accuracy while being able to produce interpretable and faithful reasoning steps. PaLI-X + VPT outperforms all existing LMMs on a wide range of visual tasks, improving performance on counting, spatial relations, and compositional reasoning tasks.  Moreover, we show that VPT is also helpful for quick adaptation on new tasks. Our experiments on content moderation show that fine-tuning LMMs with program-augmented examples is more sample efficient than traditional supervised training.

Recent advances in vision-language models (VLMs) have demonstrated striking performance on a wide range of multimodal tasks, such as visual question answering (VQA), image captioning, object recognition, and more \cite{chen2022pali, chen2023palix, chen2023pali3}.
However, despite the large strides in the field, VLMs are still lagging behind the state-of-the-art in text-only large language models (LLMs) in their ability to follow instructions provided by a user, and provide precise answers supported by explanations for open ended questions.

In an attempt to bridge this gap, recent work has tried to leverage LLMs to generate instruction-tuning data for VLMs~\cite{liu2023visual, wang2023nonintrusive, chen2023shikra, hu2022promptcap}.
For example, \otilia{which paper?} provide image captions and bounding box annotations as input to an LLM to generate sample questions and answers, which are then used to instruction-tune a VLM.
However, this approach suffers from several liabilities: 
1) LLMs are known be prone to hallucinations \otilia{CITE}, which can lead to noisy instruction-tuning data for the VLM.
2) Image captions are coarse description of images that miss important details that are necessary for solving the task. 
3) LLMs are not trained to reason with bounding boxes. As a result, these VLMs perform poorly on tasks that require fine-grained visual understanding and reasoning. 
4) Even state-of-the-art proprietary models such as GPT-4V \otilia{cite} are bad at tasks that involve counting and spatial reasoning~\cite{yang2023dawn}.

In another line of work, visual programming, a recent multimodal framework, has shown promise in conducting visual reasoning in an interpretable and compositional manner~\cite{gupta2023visprog, surismenon2023vipergpt}. Given a query, it first uses an LLM to generate a program, and then executes this program with visual modules to get the answer. Nevertheless, this framework easily fails in practice—for instance, when the program is wrong, or when a visual module make mistakes in any of the steps of the program. Moreover, visual programs cannot be trained in an end-to-end manner, so its performance is not scalable with the amount of labeled data. As a result, the performance is much lower than end-to-end systems trained with supervised learning~\cite{surismenon2023vipergpt}. In addition, it is inefficient to involve multiple steps (i.e., generating and then running programs) during inference. Ideally, a single model should directly conduct similar reasoning and yield the correct answer.

In our work, we take advantage of lessons learnt form past work: we leverage the fact that visual programs are optimal for generating multimodal instruction-tuning data, as well as take advantage of the reasoning power of LLMs.
We introduce {\em Visual Program Distillation} (VPD), a method that uses visual programming to further boost the performance and truthfulness of VLMs, enhancing their compositional and fine-grained visual reasoning ability. 
% to generate the programs, and utilizes specialized vision tools (e.g. object detection, VQA, depth estimation) to reason across modality. 
Our method is depicted in Figure~\ref{fig:method}. 
Given a query, we first generate a program that leads to the correct answer, and then transfer its execution trace into instruction-tuning data for VLMs. Compared with prior work, which uses LM and image captions to synthesize instruction-tuning data, our method has the following advantages: (1) The vision tools used in visual programs are much more powerful than image captions, and can provide more fine-grained visual information (e.g., depth of an object, relationship between bounding boxes, etc.) than LLM generated data (2) LLM-generated programs are better at tackling compositional tasks, compared with vanilla LLM generation~\cite{chen2022program}. (3) Program execution traces are more truthful and consistent than LLM generations, as shown in related works on LLMs~\cite{lyu2023faithful}. Training with program-generated data may reduce the hallucination introduced by LLM-generated data. One challenge we face is that visual programs are error-prone, as discussed earlier. To tackle with this problem, during our data synthesis process, we generate many programs from the LLM, and then filter the program by checking if the program output is correct. This approach greatly improves the data-generation efficiency, and also make our model more accurate than zero-shot visual programs.

We demonstrate the effectiveness of VPD on a wide range of tasks. Our generalist model, PaLI-X VPD (55B), sets the new state-of-the-art result on 8 classical VQA tasks and 2 zero-shot multi-model benchmarks. In the specialist setting, we conduct per-task fine-tuning on PaLI-X VPD, and shows that it outperforms the prior SoTAs set by PaLI-X. 
Human Evaluation shows that PaLI-X VPD generates more consistent and faithful rationales, compared with its counterpart trained with LM-generated data.
We also conduct these experiments on PaLI-3 (5B), showing that VPD also works for smaller-scale models. Finally, we conduct comprehensive analysis on visual programs and our method. We also discuss how to further scale up VPD framework for future work, by adding more powerful vision tools in the pipeline (e.g. segmentation), better code-generation model, and new filtering strategy that works on large-scale unlabeled images.

Our main contributions are:
\begin{enumerate}
    \item We propose Visual Program Distillation (VPD), a novel framework that distills the reasoning power of LLM-generated programs and the perception power of specialized vision tools into one vision language model (VLM).
    \item Our models trained with VPD, PaLI-3 VPD (5B) and PaLI-X VPD (55B) improves the SoTA on a broad of range of tasks, especially on tasks that requires compositional visual reasoning (e.g., counting, spatial relation).
    \item Human Evaluation shows that PaLI-X tuned with VPD generate more truthful and consistent rationales, in comparison with PaLI-X tuned with LLM-generated instruction data.
    \item We conduct comprehensive analysis on our method and visual programs, identifying limitations, and proposes future improvements.
    
\end{enumerate}

==> old/scratch.tex <==






% Needs to go in related work:

(1) The vision tools used in visual programs are much more powerful than image captions, and can provide more fine-grained visual information (e.g., depth of an object, relationship between bounding boxes, etc.) than LLM generated data (2) LLM-generated programs are better at tackling compositional tasks, compared with vanilla LLM generation~\cite{chen2022program}. (3) Program execution traces are more truthful and consistent than LLM generations, as shown in related works on LLMs~\cite{lyu2023faithful}.

==> tables/cot_vs_label.tex <==
\begin{table}[h]
\small
\centering
\caption{
Comparison between PaLI-X VPD's accuracy of directly decoding the answer v.s. using a COT to infer the answer. Here we use LLM as evaluator.
}
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{l|rr}
\toprule[1.2pt]
Dataset & Direct & COT \\
\midrule
GQA \\
OK-VQA \\
A-OKVQA MC \\
A-OKVQA DA  \\
TallyQA Simple \\
TallyQA Complex \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:statistics}
% \bottomrule
\vspace{-3mm}
\end{table}

==> tables/visual_program_filtering.tex <==
\begin{table}[h]
\small
\centering
\caption{
Ratio of programs kept after filtering.
}
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{l|rr}
\toprule[1.2pt]
Dataset & success@1 & success@5 \\
\midrule
GQA & 43.7 & 63.7 \\
OK-VQA & 57.2 & 76.6 \\
A-OKVQA & 47.0 & 68.7 \\
TallyQA & 63.4 & 69.7 \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:statistics}
% \bottomrule
\vspace{-3mm}
\end{table}

==> tables/vpd_vs_program.tex <==
\begin{table}[h]
\small
\centering
\caption{
Comparison between visual programs and PaLI-X VPT on the validation sets. 
}
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{l|rr}
\toprule[1.2pt]
Dataset & Program & PaLI-X VPT \\
\midrule
GQA & 41.1 & 64.9 \\
OK-VQA & 50.2 & 64.6 \\
A-OKVQA MC & 50.7 & 84.5 \\
A-OKVQA DA & 48.3 & 62.7 \\
TallyQA Simple & 72.3 & 86.2 \\
TallyQA Complex & 51.8 & 76.6 \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:statistics}
% \bottomrule
\vspace{-3mm}
\end{table}
